Focus on the Common Good: Group Distributional Robustness Follows

We consider the problem of training a classification model with group annotated training data. Recent work has established that, if there is distribution shift across different groups, models trained using the standard empirical risk minimization (ERM) objective suffer from poor performance on minority groups and that group distributionally robust optimization (Group-DRO) objective is a better alternative. The starting point of this paper is the observation that though Group-DRO performs better than ERM on minority groups for some benchmark datasets, there are several other datasets where it performs much worse than ERM. Inspired by ideas from the closely related problem of domain generalization, this paper proposes a new and simple algorithm that explicitly encourages learning of features that are shared across various groups. The key insight behind our proposed algorithm is that while Group-DRO focuses on groups with worst regularized loss, focusing instead, on groups that enable better performance even on other groups, could lead to learning of shared/common features, thereby enhancing minority performance beyond what is achieved by Group-DRO. Empirically, we show that our proposed algorithm matches or achieves better performance compared to strong contemporary baselines including ERM and Group-DRO on standard benchmarks on both minority groups and across all groups. Theoretically, we show that the proposed algorithm is a descent method and finds first order stationary points of smooth nonconvex functions.

==> attic/ablation.tex <==
\section{Ablation Analysis}
\todo[inline]{Revisit}
Figure~\ref{fig:ablation:spusimple},~\ref{fig:ablation:noisesimple} compares {\cg} shown in~\eqref{eqn:cg} with two of its variants on the two simple settings. We can directly optimize the objective shown in~\eqref{eqn:cgerm} without finding an optimal training weights which we refer to as {\cgerm}. Instead of the sq-root scaling of the losses, we can obtain the training weights using a simpler form shown in~\eqref{eqn:cgsimple} that we refer to as {\cgsimple}.
{\cg} emphasizes the clean-majority better in Spu-Simple setting and is more robust to noisy group in the Noisy-Simple setting. 
Table~\ref{tab:ablation:rmnist} compares the variants on Rotated MNIST setting. The trend remains intact even on this setting.

\begin{table}[htb]
    \centering
    \begin{tabular}{|c|r|}
    \hline
    \thead{Alg. $\downarrow$} & \thead{Test Metric}\\\hline
        {\cgerm} &  90.0 (0.5), 80.8 (1.2)\\
        {\cgsimple} & 92.1 (0.2), 84.6 (0.9) \\
        {\cg} & 92.1 (0.6), 85.0 (0.7)\\\hline
    \end{tabular}
    \caption{Ablation analysis on Rotated MNIST}
    \label{tab:ablation:rmnist}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{plots/spu-simple_all_0.pdf}
    \caption{Training weight dynamics for {\cg}, {\cgsimple}, {\cgerm}, {\dro} in that order from left to right on Spu-Simple generative setting. {\cg} promotes the clean majority more than its variants: {\cgsimple}, {\cgerm}.}
    \label{fig:ablation:spusimple}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{plots/noisy-simple_all_0.pdf}
    \caption{Training weight dynamics for {\cg}, {\cgsimple}, {\cgerm}, {\dro} in that order from left to right on Noisy-Simple generative setting. {\cg} is more robust than its variants to the presence of the noisy group due to combined effect of square-root loss and transferability correction.}
    \label{fig:ablation:noisesimple}
\end{figure}

==> attic/intro.tex <==
Machine Learning (ML) algorithms are increasingly prevalent in several domains including applications that require critical decision making such as in health care. Large deep learning based ML algorithms are found to generalize surprisingly well despite the large model complexity. However, several recent findings highlight the drawbacks in the seemingly effective models. The problem is loosely referred to as the ``shortcuts'' in learning. That is, the deep feature learners focus only on shortcuts (simplest explanation) even in the presence of less noisy but complex features~\citep{ShahTR20}. Prediction based on such dataset specific shortcuts lead to poor performance when evaluating in the wild~\citep{DegraveRadiology21,Geirhos20}.
Shortcut explanations could leak in to the training data for a variety of reasons~\citep{Geirhos20} and if present defocuses the expected learning task. Handling this challenge would require a concerted change in the training ecosystem of the ML algorithms, from how we create data~\citep{KaushikCfactual19}, what risk we minimize~\citep{ArjovskyIRM19,Sagawa19,Ahmed21}, and how we encode inductive biases that enable human-like learning~\citep{Geirhos18}. A slightly less ambitious, but challenging, problem is when examples that disagree with the shortcut are represented during training, albeit with a small size, and we are provided per-example annotations on whether it agrees or disagrees with the shortcut. In this problem setting, we can focus solely on the training risk aspect of the shortcut problem. Such highly correlated but nuisance features (shortcut explanation) are also referred to as spurious correlations and the corresponding training objective of ignoring them the spurious correlation avoidance problem in the literature.  

\citet{Sagawa19} popularized the spurious correlations problem (SC), in the context of high capacity model training, where examples are annotated with a group label depending on whether or not it confirms with the spurious feature, both during train and evaluation. 
% The nature of grouping is such that when the model relies on the spurious correlation, the performance of at least one of the groups is worser than otherwise. As a result, the worst-group accuracy metric is
The problem mandates uniform performance on all the groups, in fact a model is evaluated by the worst group performance metric. The basis for grouping often has physical interpretation owing to its practical usage, such as protected attributes from fairness literature. For example, we expect gender classification system to perform equally well on all the skin colors (represented in the training set), the objective then is to have comparable performance across skin color (protected attribute) identifying groups. When the group sizes are disproportionate and when there exists a simpler hypothesis (shortcut) on the majority group that negatively interferes with the minority group, the generalization performance of the minority group suffers greatly. A typical example of negative interference is an animal classification task when the majority group are images with {\it camel} in a desert and {\it cow} in a meadow, it is likely that the learning model picks on the background features for the animal type. Such a model will perform poorly when {\it camel} is found in a meadow and vice-versa. 
% We say the spurious correlation problem is less ambitious because it specifies the negatively interfering groups in the training data which could be unavailable in some applications. 
The spurious correlation problem is related to the ``domain generalization'' (DG) problem. The goal of DG is to learn a hypothesis that generalizes beyond the finite and possibly few train domains.
The aspect of training on multiple domains/groups is common between the SC and DG problems, while SC evaluates only over the seen train domains, DG evaluates on both seen and unseen domains. 

The SC problem is acute when the ratio of number of examples that disagree with the spurious feature to the number that agree is very small~\citep{SagawaExacerbate20}. Since the problem is rooted in the under-representation of the sub-population that is negatively affected by the spurious correlation, a simple baseline is minority group up-weighting. This baseline, however, carries the risk of overfitting on the minority group and does not serve to counter the spurious correlations. We could regularize strongly or stop training early and alleviate the minority overfitting problem to some extent, such an estimator runs the problem of under-fitting on the majority and could still be sub-optimal. \citet{SagawaExacerbate20} recommends under-sampling the majority rather than over-sampling the minority, this baseline too has the majority under-fitting problem. \citet{MenonOverparam21} argues that majority under-sampling only when fine-tuning the final classification layer of a model trained only on the majority groups is equally effective. 

\citet{Sagawa19} proposed a loss value based reweighting strategy. It extends and studies an existing Distributionally Robust Optimization (DRO)~\citep{duchi18} objective to the group setting called {\dro}. Their algorithm at each step trains over groups with (soft-)maximum loss. {\dro} by only training on the worst loss group avoids overfitting on any of the train groups and is found to have been more or equally effective than any other group weighting strategy so far. When a group incurs high training loss due to label or input noise, {\dro} in such a case would overly focus on the noisy groups. Even when the noise levels across the groups is comparable, some groups might transfer better to the minority than others, it is not clear if it is a good strategy to focus on the worst group instead of on the groups that transfer well to all the groups. The optimal weighting strategy is often unknown and different methods are evaluated based on the final performance. We will look at synthetic multi-domain training settings where the optimal weighting strategy is known. We highlight some of the drawbacks of the existing methods qualitatively with the aid of these synthetic settings.

The difficulty of the SC problem is a manifestation of a more general challenge of training on heterogeneous domains. The heterogeneity could arise due to (1) non-uniform training sizes (2) varying difficulty or noise level (3) non-uniform inter-domain interactions, i.e. some domain pairs transfer positively and some negatively. Each of the afore mentioned causes lead to different training loss patterns. Non-uniform training sizes lead to different learning paces, i.e. the loss on the minority groups converge faster than the majority groups. Varying difficulty or noise levels lead to disproportionately scaled loss values and when using vanilla gradient descent method on the cumulative loss, the gradient is dominated by the contribution from the difficult group(s) which is undesired when the difficulty arises from input/label ambiguity/noise. Non-uniform inter-domain interactions cause complex coupling of the training losses, if two groups transfer positively then training on one decreases the loss on both, if on the other hand interact negatively then training on one spikes the other group. The existing methods focus only on heterogeneity due to non-uniform training sizes. {\ermuw} upweighs the minority group in an attempt to equalize training representation, {\dro} adopts a learning strategy that induces uniform learning pace. We design an algorithm that is robust to all the three aspects of heterogeneity.

\todo[inline]{Will revise the following once we finalize our story.}
We set the objective to cumulative square-root loss instead of cumulative loss and obtain the training weights at every update step from inner loop maximization of the total loss decrement. We discuss more details in Section~\ref{sec:method}. We demonstrate the robustness of our algorithm in synthetic (Section~\ref{sec:qua}) as well as real world settings (Section~\ref{sec:expt}). Our contributions are listed below.

\begin{itemize}
\item {We identify multiple facets of training on heterogeneous domains that are not addressed in the earlier work.}
\item {Our synthetic setting serves as a testbed for qualitative evaluation of the existing methods.}
\item {We present an algorithm that is robust to all the identified aspects of heterogeneous domain training.}
\item {We demonstrate effectiveness of our algorithm on 5 synthetic and 5 real-world datasets.}
\end{itemize}

==> old.tex <==
\section{Motivation}

ERM's gradient update ($g_c$) when training on multiple groups can be seen as the minimizer of the optimization equation below.

\begin{align*}
g_c = \argmin_g \sum_{i=1}^n(g_i-g)^2
\end{align*}

That is, the gradient update ($g_c$) needs to be aligned both in magnitude and direction with all the domain gradients. When the domains are heterogeneous, they differ in: size, difficulty, noise levels; as a result, the domain gradients vary in their magnitude. The gradient update obtained from optimization expression above could focus only on a subset of the domains, leading to disparate domain level performance levels. Instead, we argue that the gradient update be only aligned in direction but not the magnitude of the domain gradients. The corresponding optimization equation with a domain scaling parameter: $\alpha \in \mathbb{R}_{+}^n$ is shown below.

\begin{align}
  g_c &= \argmin_g\min_\alpha \sum_{i=1}^n (g_i - \alpha_ig)^2\\
  &=\arg\min_g\min_\alpha \frac{1}{2}\|\alpha\|_2^2\|g\|^2 - g^T(\sum_i\alpha_ig_i)\\
  &\textrm{with the constraint $\alpha>0$}\nonumber
\end{align}

The optimal value of $\alpha$ for a given value of g is such that:

\begin{align*}
    \alpha^*_i &\propto g^Tg_i + \lambda_i\quad \forall i\in [n]\\
    &\text{(for some $\lambda_i\geq 0$ such that the right hand side is positive.)}
\end{align*}

The optimal value of $g$ for a given value of $\alpha$ is:

$$
g = \sum_i \alpha_ig_i/\|\alpha\|^2
$$

We alternate the updates on $\alpha$ and $g$ to obtain the following expressions for the gradient update at $t^{th}$ step. 

\begin{align*}
g &= \sum_i\alpha^{(t-1)}_ig_i \\
\alpha_i^{(t)} &= [\sum_j \alpha_j^{(t-1)}g^T_jg_i]_+\\
g^{(t)} &= \sum_i \alpha_i^{(t)}g_i
\end{align*}

\subsection{Alternate}

The gradient update for ERM is the solution to the following optimization. 

\begin{align}
\argmax_g  \sum_i g^Tg_i - \frac{1}{2}\|g\|^2
\end{align}

For that of CG is the following:

\begin{align}
    \argmax_g &\sum_i g^Tg_i \\
    &\text{such that } g=\sum_i\lambda_i g_i, \lambda\geq 0, \sum_i \lambda_i = n 
\end{align}

Notice that the optimization expression for CG is missing the minimization of gradient norm term. In other words, CG finds an update in the convex hull that has large norm and is close to the cumulative gradient: $\sum_i g_i$.

Large gradient norm is an outcome of excluding gradients from conflicting groups from the update: $\sum_i \alpha_ig_i$.

\iffalse
\subsection{Meta-objective}

We wish to find a training loss weights ($\alpha$) such that we decrease the cumulative loss on all the groups maximally. The meta-objective and the optimal solution is obtained using the following steps. Let $l_i, g_i$ denote the loss, gradient of the i$^{th}$ group. G denotes the $m\times m$ matrix that contains all pairwise dot products of the m groups such that $G_{ij}=g_i^Tg_j$.

\begin{align}
\alpha^* &= \max_\alpha \sum_i l_i(\theta) - l_i(\theta - \eta\sum_j\alpha_jg_j) \label{eqn:cgsimple}\\
&\text{Using first order Taylor expansion}\nonumber\\
 &= \max_\alpha \sum_i [g_i^T \sum_j\alpha_j g_j]\nonumber\\
&=\max_\alpha \sum_i\sum_j \alpha_j<g_i, g_j>\nonumber\\
&=\max_\alpha \sum_i G[i]\alpha = \max_\alpha \mathbf{1}^TG\alpha = \max_\alpha \alpha^TG^T\mathbf{1}\nonumber\\
&=\max_\alpha \sum_i \alpha_iG[i]^T\mathbf{1}\quad \alpha>0, \alpha\mathbf{1}=1\nonumber\\
&\textrm{Exponential gradient ascent on $\alpha$ gives}\nonumber\\
\alpha_i\propto & \alpha_i\exp(\eta_\alpha G[i]^T\mathbf{1})\quad\forall i
\end{align}

But is $\Delta l_{ij}$, i.e. loss decrement on i$^{th}$ group using j$^{th}$ group's gradient proportional to $g_i^Tg_j$? The actual update we are using will follow if we assume $\Delta l_{ij}=\sqrt{l_i}\sqrt{l_j}\text{cosine-sim}(g_i, g_j)$.

{\it This parameter update can also be argued from common-specific decomposition: identify common component from the negative specific components, meta-learning: update with that maximum loss decrement.}
\fi
